UnProjection: Leveraging Inverse-Projections for Visual Analytics of High-Dimensional Data

Projection techniques are often used to visualize high-dimensional data, allowing users to better understand the overall structure of multi-dimensional spaces on a 2D screen. Although many such methods exist, comparably little work has been done on generalizable methods of inverse-projection -- the process of mapping the projected points, or more generally, the projection space back to the original high-dimensional space. In this paper we present NNInv, a deep learning technique with the ability to approximate the inverse of any projection or mapping. NNInv learns to reconstruct high-dimensional data from any arbitrary point on a 2D projection space, giving users the ability to interact with the learned high-dimensional representation in a visual analytics system. We provide an analysis of the parameter space of NNInv, and offer guidance in selecting these parameters. We extend validation of the effectiveness of NNInv through a series of quantitative and qualitative analyses. We then demonstrate the method's utility by applying it to three visualization tasks: interactive instance interpolation, classifier agreement, and gradient visualization.

==> sec-motivation.tex <==
\section{Motivation}
\label{sec:motivation}
%
Projections from a high-dimensional space down to two dimensions enable the visual inspection of high-dimensional data on a flat screen.
%
Inverse-projections methods such as iLamp\cite{amorim:2012:ilamp} and RBF\cite{amorim:2015:rbf} have recently been offered as techniques for providing a better understanding of those projections.
%
They've been evaluated primarily based on quantitative error and scalability measures.
%
For example, let $\mathcal{D}$ be the data space, with the dataset $\bm{X}\subset \mathcal{D}$\footnote{In this paper bold lowercase will indicate a vector, and bold uppercase a matrix.}.
%
Let $p:\mathcal{D} \rightarrow \mathbb{R}^2$ be the projection and $b:\mathbb{R}^2 \rightarrow \mathcal{D}$ be the inverse-projection.
%
Mean Squared Error can be expressed in terms of the distances between points in the original data and their reconstructions, and a low mean-square error (MSE) can be a way of evaluating inverse-projections.
%
\[
    MSE(b, p, \bm{X}) = \frac{1}{n}\sum_{i=1}^{n}{dist(\bm{x}_i, b \circ p (\bm{x}_i))^2}
\]
%
This quantitative evaluation is used to validate both the projection $p$ and the inverse-projection $b$.
%
For the projection, we want this error to be small because it means that the projection maintained much of the information of the data $\bm{X}$, and that the projected space can serve as a proxy for the high dimensional space without much loss.
%
And for the inverse-projection $b$, we want this error to be small because it validates that the technique used to generate the inverse-projection was accurate.
%

%
However, this evaluation is missing a crucial aspect of the use of the projected space.
%
The tasks that the projected space enables don't only depend on the projected points, but also the space in between.
%
The exploration of this projected space has previously been used to generate graph layouts\cite{kwon:2020:deep_generative_graphs} or even generate candidates for the discovery of new molecules\cite{gomez:2018:chem_design_using_back_projection}.
%
The region outside of the projected points but still in the projection can be expressed as the image of $\mathcal{D} \setminus X$ over $p$, which we'll express as $p(\mathcal{D} \setminus \bm{X})$.
%
The performance of the projection in this space is entirely missed by the mean square error: it tells us only about $p(\bm{X})$.
%

%
However, there is no ground truth for the $p(\mathcal{D} \setminus \bm{X})$ because no inverse for $p$ can exist if the dimensionality of $D$ is greater than 2.
%
In this paper, we analyze different properties of the inverse-projection $b$ that can help evaluate $p(\mathcal{D} \setminus \bm{X})$, i.e. the parts of the projected space outside of the projected points.  
%
In particular, we look at three properties.
%
\begin{itemize}
    \item $b (\mathbb{R}^2\setminus p(\bm{X}))$ \textbf{Dynamic Imputation:} We look at the inverse-projections of the area outside of projected points in the 2D projection.
    %
    By dynamically exploring these points and seeing how they impute between ground truth, the user can get a sense of where major changes occur in the projected space.
    %

    %
    \item $f \circ b \circ p(\mathcal D)$ \textbf{Preservation of Functions and Classifier Agreement:} A very typical technique for mathematical interpretation of mappings is to observe what properties of a function on the domain are preserved in the image of the mapping.
    %
    In Rodrigues et al.'s dense maps\cite{rodrigues:2019:classifier_boundaries}, the function is the label function: the projected space is colored by how a classifier divides up the space.
    %
    We instead look at a different function, classifier agreement, to parcel up the space into connected regions that reflect where changes occur in the data with respect to classifier agreement.
    %

    %
    \item $\partial b \circ p (\mathcal D)$ \textbf{Gradient-Map Visualizations:} We look at the gradient of the inverse-projections to see which regions of the projected space were stretched the most to fit into the 2D screen. %
    This reveals locations in the projected space where distances are least reliable.
    %
\end{itemize}
%
In this paper, we use deep learning as a flexible inverse-projection technique, as suggested by Espadoto et al.\cite{espadoto:2019:nn_inv}.
%
It has been shown to produce accurate inverse-projections in terms of MSE in an efficient manner.
%
In addition, it is a differentiable function, making the gradient easy to calculate.
%
We inspect these three properties of projections of various datasets, paying special attention to datasets whose topological properties are well known, such as spheres or MNIST, because these topological properties can stand in as validation in light of the lack of ground truth for the projected space.
%
